A Tight Lower Bound for Streett Complementation

Finite automata on infinite words ($\omega$-automata) proved to be a powerful weapon for modeling and reasoning infinite behaviors of reactive systems. Complementation of $\omega$-automata is crucial in many of these applications. But the problem is non-trivial; even after extensive study during the past four decades, we still have an important type of $\omega$-automata, namely Streett automata, for which the gap between the current best lower bound $2^{\Omega(n \lg nk)}$ and upper bound $2^{\Omega(nk \lg nk)}$ is substantial, for the Streett index size $k$ can be exponential in the number of states $n$. In arXiv:1102.2960 we showed a construction for complementing Streett automata with the upper bound $2^{O(n \lg n+nk \lg k)}$ for $k = O(n)$ and $2^{O(n^{2} \lg n)}$ for $k=\omega(n)$. In this paper we establish a matching lower bound $2^{\Omega(n \lg n+nk \lg k)}$ for $k = O(n)$ and $2^{\Omega(n^{2} \lg n)}$ for $k = \omega(n)$, and therefore showing that the construction is asymptotically optimal with respect to the $2^{\Theta(\cdot)}$ notation.

==> construction.tex <==
\section{Construction of $Q$-Words}
\label{sec:construction}

In this section we prove Theorem~\ref{thm:existence}. Recall that we need a construction to simultaneously satisfy all properties in Definition~\ref{def:Q-word}, which are parameterized with pairs of states (Condition~\eqref{en:Q-word-1}) or states (Condition~\eqref{en:Q-word-2}). The idea is to concatenate a sequence of finite $\Delta$-graphs, each of which satisfies the properties with respect to a specific pair of states or a specific state. With the help of the bypass track ($t$-track), properties associated with each individual subgraph are all preserved in the final concatenation, giving us a desired $Q$-word.

Let $f=\langle r,h \rangle$. $\scrG_{f}$ divides into two sequential subgraphs $\scrG_{r}$ and $\scrG_{h}$, which satisfy Properties~\eqref{en:Q-word-1} and~\eqref{en:Q-word-2}, respectively. Properties~\eqref{en:Q-word-3} and~\eqref{en:Q-word-4} are obvious once the final construction is shown. As stated earlier, Property~\eqref{en:Q-word-1} and Property~\eqref{en:Q-word-2} are orthogonal; Property~\eqref{en:Q-word-1} only relies on $R$-rankings and Property~\eqref{en:Q-word-2} only relies on $H$-rankings. We call a finite $\Delta$-graph whose every level is ranked by the same $R$-ranking, an \emph{$R$-word} if it satisfies Properties~\eqref{en:Q-word-1},~\eqref{en:Q-word-3} and~\eqref{en:Q-word-4}. Similarly, a finite $\Delta$-graph whose every level is ranked by the same $H$-ranking, is called an \emph{$H$-word} if it satisfies Properties~\eqref{en:Q-word-2},~\eqref{en:Q-word-3} and~\eqref{en:Q-word-4}. As $Q$-words, $H$-words (resp. $R$-words) are not uniquely determined by $H$-rankings (resp. $R$-rankings). Nevertheless, all $H$-words (resp. $R$-words) corresponding to a specific $h$ (resp. $r$) serve the construction purpose equally well, and hence we simply name an arbitrarily chosen one by $\scrG_{h}$ (resp. $\scrG_{r}$). Theorem~\ref{thm:existence} builds on Lemmas~\ref{lem:R-word} and~\ref{lem:H-word}.

\begin{lemma}[$R$-Word]
\label{lem:R-word}
An $R$-word exists for every $R$-ranking.
\end{lemma}

\begin{example}[$R$-Word]
\label{ex:R-word}
Let us revisit Example~\ref{ex:Q-word}. In Figure~\ref{fig:Q-word}, the $R$-word $\scrG_{r}$ consists of two parts: $\scrG^{(1)}_{r}$ (level $0$ to level $3$) and $\scrG^{(2)}_{r}$ (level $3$ to $6$). For Property~\eqref{en:Q-word-1} with respect to $q_{2}$ and $q_{1}$, we can obtain the desired $\varrho_{2, 1}$ as follows. In $\scrG^{(1)}_{r}$, $\varrho_{2, 1}$ starts from $\langle q_{2}, 0 \rangle$, visits $\langle b_{1}, 1 \rangle$, $\langle b_{2}, 2 \rangle$ and then $\langle q_{0}, 3 \rangle$. In $\scrG^{(2)}_{r}$, $\varrho_{2, 1}$ continues from $\langle q_{0}, 3 \rangle$, visits $\langle b_{1}, 4 \rangle$, $\langle b_{2}, 5 \rangle$ and lands at $\langle q_{1}, 6 \rangle$. For Property~\eqref{en:Q-word-1} with respect to $q_{0}$ and $q_{1}$, we can obtain the desired $\varrho_{0, 1}$ as follows. In $\scrG^{(1)}_{r}$, $\varrho_{0, 1}$ starts from $\langle q_{0}, 0 \rangle$, passes through $\scrG^{(1)}_{r}$ via $q_{0}$-track until it reaches $\langle q_{0}, 3 \rangle$ from where it visits $\langle b_{1}, 4 \rangle$, $\langle b_{2}, 5 \rangle$ and lands at $\langle q_{1}, 6 \rangle$.
\end{example}

\begin{lemma}[$H$-Word]
\label{lem:H-word}
An $H$-word exists for every $H$-ranking.
\end{lemma}

\begin{example}[$H$-Word]
\label{ex:H-word}
Let us revisit Example~\ref{ex:Q-word}. In Figure~\ref{fig:Q-word}, the $H$-word $\scrG_{h}$ consists of three parts: $\scrG^{(1)}_{h}$ (level $6$ to level $12$), $\scrG^{(2)}_{h}$ (level $12$ to level $18$), and $\scrG^{(3)}_{h}$ (level $18$ to level $24$). Let us take a look the paths $\varrho_{h}$ and $\varrho_{h'}$ (in $\scrG^{(1)}_{h}$) defined in Example~\ref{ex:Q-word}. The path $\varrho_{h}$ (marked green except the last edge) starts at $\langle q_{1}, 12 \rangle$, visits $\langle b_{2}, 13 \rangle$ and $\langle g_{1}, 14 \rangle$, and enters $t$-track at $\langle t, 15 \rangle$. It continues on $t$-track till reaching $\langle t, 17 \rangle$, and then takes $\langle \langle t, 17 \rangle, \langle q_{1}, 18 \rangle \rangle$ (marked blue) to the end. The path $\varrho_{h'}$ (marked red except the last edge) starts at $\langle q_{1}, 12 \rangle$, takes $q_{1}$-track to reach $\langle q_{1}, 15 \rangle$, from where it visits $\langle g_{2}, 16 \rangle$ and then enters $t$-track at $\langle t, 17 \rangle$. Same as $\varrho_{h}$, $\varrho_{h'}$ returns to $q_{1}$-track via $\langle \langle t, 17 \rangle, \langle q_{1}, 18 \rangle \rangle$.
\end{example}

\begin{varthm}{\ref{thm:existence}~($Q$-Words).}
A $Q$-word exists for every $Q$-ranking.
\end{varthm}
\begin{proof}
By Lemmas~\ref{lem:R-word} and~\ref{lem:H-word}, we have $\scrG_{r}$ and $\scrG_{h}$ as an $R$-word and an $H$-word, respectively. The desired $Q$-word $\scrG$ is just $\scrG_{r} \cat \scrG_{h}$. Properties~\eqref{en:Q-word-3} and~\eqref{en:Q-word-4} follow immediately because they hold both in $\scrG_{r}$ and $\scrG_{h}$.

Let $\varrho^{r}_{i, i'}$ be the full path in $\scrG_{r}$ that satisfies Property~\eqref{en:Q-word-1} for $q_{i}$ and $q_{i'}$ where $i, i' \in [n]$ and $r(q_{i}) > r(q_{i'})$, and $\varrho^{h}_{i', k}$ the full path in $\scrG_{h}$ that satisfies Property~\eqref{en:Q-word-2} (with respect to $q_{i'}$ and index $k$). Then $\varrho^{r}_{i, i'} \cat  \varrho^{h}_{i', k}$ is the path that Property~\eqref{en:Q-word-1} requires for vertex pair $q_{i}$ and $q_{i'}$.

Let $i \in [n]$ and $j \in I$. Let $\varrho^{r}_{i,i}$ be the full $q_{i}$-track in $\scrG_{r}$, and $\varrho^{h}_{i, j}$ the full path in $\scrG_{h}$ that satisfies Property~\eqref{en:Q-word-2} (with respect to vertex $q_{i}$ and index $j$). Then in $\scrG$, for each $q \in Q$, we have $k$ full paths $\varrho^{r}_{i, i} \cat \varrho^{h}_{i, j}$ ($j \in I$), which takes care of the existence part of Property~\eqref{en:Q-word-2}. The exactness part follows from the exactness part of Property~\eqref{en:Q-word-2} for $\scrG_{h}$, and the fact that for each $i \in [n]$, $\varrho^{r}_{i,i}$ is unique in $\scrG_{r}$.
\end{proof} 
